Near-optimal Assembly for Shotgun Sequencing with Noisy Reads

Recent work identified the fundamental limits on the information requirements in terms of read length and coverage depth required for successful de novo genome reconstruction from shotgun sequencing data, based on the idealistic assumption of no errors in the reads (noiseless reads). In this work, we show that even when there is noise in the reads, one can successfully reconstruct with information requirements close to the noiseless fundamental limit. A new assembly algorithm, X-phased Multibridging, is designed based on a probabilistic model of the genome. It is shown through analysis to perform well on the model, and through simulations to perform well on real genomes.

==> draftBackUp.tex <==


\section{Extension to handle insertion/deletion
noise}

Most of the procedures implemented in the prototype assembler under
the substitution noise model can be readily generalized to handle
indel noise. We note that one non-trivial generalization is the way
that we form the noisy De Bruijn graph for K-mer clusters. In particular,
we first compute the pairwise overlap alignment among reads, then
use the overlap alignment to group K-mers into clusters. Subsequently,
we link successive cluster of K-mers together as we do in Alg \ref{alg:Noisy-Multi-Bridging-1}.
An illustration is shown in Fig \ref{fig:Form-K-mer-Clusters}. However,
due to the noise being indel in nature, the edges in the noisy De
Bruijn graph may point in the wrong direction as shown in Fig \ref{fig:Abnormalty-in-Noisy(indel)}.
In order to handle this, we tranverse the graph and remove such abnormalty
when they are detected. 

We also implemented a generalized version of the prototype assembler to handle indel noise
and we test it on synthetic reads sampled from synthetic genome. Simulation
results are summarized in Table \ref{tab:Simulation-Results-for}
where $p_{i},p_{d}$ are insertion probability and deletion probability and
rate is the number of successful reconstruction in 10 rounds.

Although the prototype assembler is functional and can produce the results presented in this paper, we note that the assembler we have at the point of writing is only a prototype version. We are 
in the process of transforming the prototype assembler into a practical assembler to facilitate sequencing using 
PacBio indel noise corrupted reads to finish more real genomes. 

\begin{table}
\begin{centering}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline 
$G$  & $p_{i}$  & $p_{d}$  & $\frac{NL}{G}$  & $L$  & $l_{simple}^{approx}$  & $l_{crit}^{approx}$  & $l_{crit}^{exact}$  & $\frac{N}{N_{noiseless}}$  & $\frac{L}{l_{crit}^{exact}}$ & Rate\tabularnewline
\hline 
\hline 
10000 & 1.5\%  & 1.5\%  & 15.1 & 200 & 500 & 200 & 100 & 1.81 & 2  & 9/10\tabularnewline
\hline 
10000 & 1.5\%  & 1.5\%  & 15.6 & 180 & 500 & 200 & 100 & 1.85 & 1.8 & 9/10\tabularnewline
\hline 
10000 & 1.5\%  & 1.5\%  & 16.3 & 160 & 500 & 200 & 100 & 1.81 & 1.6 & 9/10\tabularnewline
\hline 
\end{tabular}
\par\end{centering}

\caption{\label{tab:Simulation-Results-for}Simulation Results for indel treatment}
\end{table}


\newpage{}  \bibliographystyle{plain}

==> related_work.tex <==
%
% summary and outline 
%
%\subsection*{Related Work}

All assemblers must somehow address the problem of resolving noise in the reads in the genome reconstruction -- however, the traditional approaches to measuring assembly performance makes quantitative comparisons challenging for unfinished genomes~\cite{NM2011}.  In most cases, the heart of the assembly problem lies in processing of the assembly graph, as in  \cite{zerbino2008velvet,gnerre2011high,simpson2012efficient}.  A common strategy for dealing with ambiguity from the reads lies in filtering the massively parallel sequencing data using the graph structure prior to traversing possible assembly solutions.  In the present work, however, we are focused on the often overlooked goal of optimal data efficiency.  Thus, to the extent possible we distinguish between the read error and the inherent ambiguity associated with the shotgun sampling process.  The proposed  X-phased Multibridging assembler thus adds information to the assembly graph from analyzing the underlying reads to resolve assembly graph ambiguities in a novel way.


%@article{NM2011,
%    author = {Narzisi, Giuseppe AND Mishra, Bud},
%    journal = {PLoS ONE},
%    publisher = {Public Library of Science},
%    title = {Comparing De Novo Genome Assembly: The Long and Short of It},
%    year = {2011},
%    month = {04},
%    volume = {6},
%    url = {http://dx.doi.org/10.1371%2Fjournal.pone.0019175},
%    pages = {e19175},
%    number = {4},
%    doi = {10.1371/journal.pone.0019175}
%}        




